Do fragmentation and accretion affect the stellar Initial Mass Function?

While the stellar Initial Mass Function (IMF) appears to be close to universal within the Milky Way galaxy, it is strongly suspected to be different in the primordial Universe, where molecular hydrogen cooling is less efficient and the gas temperature can be higher by a factor of 30. In between these extreme cases, the gas temperature varies depending on the environment, metallicity and radiation background. In this paper we explore if changes of the gas temperature affect the IMF of the stars considering fragmentation and accretion. The fragmentation behavior depends mostly on the Jeans mass at the turning point in the equation of state where a transition occurs from an approximately isothermal to an adiabatic regime due to dust opacities. The Jeans mass at this transition in the equation of state is always very similar, independent of the initial temperature, and therefore the initial mass of the fragments is very similar. Accretion on the other hand is strongly temperature dependent. We argue that the latter becomes the dominant process for star formation efficiencies above 5 - 7 %, increasing the average mass of the stars.

==> Comments--Response <==
Responding your comments:

1.	The title has been adjusted now.

2.	Ralf Klessen as co-author has been introduced now.

3.	word corrected in the abstract.

4.	\citep used now for the Klessen and Bovino reference.

5.	I now cited Paul Clark and the related text is shown in bold letters.

  

